Gradient Frequency Modulation for Visually Explaining Video Understanding Models

In many applications, it is essential to understand why a machine learning model makes the decisions it does, but this is inhibited by the black-box nature of state-of-the-art neural networks. Because of this, increasing attention has been paid to explainability in deep learning, including in the area of video understanding. Due to the temporal dimension of video data, the main challenge of explaining a video action recognition model is to produce spatiotemporally consistent visual explanations, which has been ignored in the existing literature. In this paper, we propose Frequency-based Extremal Perturbation (F-EP) to explain a video understanding model's decisions. Because the explanations given by perturbation methods are noisy and non-smooth both spatially and temporally, we propose to modulate the frequencies of gradient maps from the neural network model with a Discrete Cosine Transform (DCT). We show in a range of experiments that F-EP provides more spatiotemporally consistent explanations that more faithfully represent the model's decisions compared to the existing state-of-the-art methods.

==> images/fig_table.tex <==
\newcommand\figcaption{\def\@captype{figure}\caption}
\newcommand\tabcaption{\def\@captype{table}\caption}
\makeatother

\begin{figure}[tb]
	\centering
		\begin{minipage}{0.4\textwidth}
			\centering
			\begin{tabular}{|l|rl|}
				\hline
				\bf Model & \bf $F_1$ &  \\ 
				\hline
				\quad-- CCCC    & 70 &  \\
				\quad-- DDDD     & 72 &  \\			
				\quad-- AAAA        & 71 &  \\
				\quad-- BBBB     & 68  &  \\
				\hline
			\end{tabular}
			\tabcaption{Ablation study of XXX.}
			\label{tab:ablation}
		\end{minipage}
	\hspace{0.5in}
		\begin{minipage}[h]{0.45\linewidth}
			\centering
			\includegraphics[scale=0.45]{xxx.pdf}
	        \figcaption{$F_1$ variation with XXX}
	        \label{fig:layers}
		\end{minipage}%
\end{figure}

==> images/r3d_ucf101.tex <==
\newcommand{\framewidth}{0.13\linewidth}
\newcolumntype{T}{>{\tiny}l}
\newcolumntype{H}{>{\Huge}l}

\begin{figure*}[t]
\footnotesize
\centering
\renewcommand{\tabcolsep}{0.7pt} %
\begin{tabular}{>{\scriptsize}ccccccccc}
% & 29, prob:[0.63] & 14, prob:[0.0004] & 99, prob:[0.374] & 4, prob:[0.872] &
% \\
\parbox[c]{4mm}{\multirow{1}{*}[3.0em]{\rotatebox[origin=c]{90}{Input}}} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-2.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-3.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-6.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-7.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-8.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-10.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-12.png} &

% \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-8.png}
\parbox[c]{4mm}{\multirow{1}{*}[3.5em]{\rotatebox[origin=c]{90}{FG, [0.63]}}}
\\
\parbox[c]{4mm}{\multirow{1}{*}[5.5em]{\rotatebox[origin=c]{90}{Grad-CAM\cite{grad-cam}}}} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gc/floorGymnastics_g01_c01[49-64]-[frame4]2.jpg} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gc/floorGymnastics_g01_c01[49-64]-[frame5]3.jpg} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gc/floorGymnastics_g01_c01[49-64]-[frame8]6.jpg} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gc/floorGymnastics_g01_c01[49-64]-[frame9]7.jpg} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gc/floorGymnastics_g01_c01[49-64]-[frame10]8.jpg} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gc/floorGymnastics_g01_c01[49-64]-[frame11]10.jpg} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gc/floorGymnastics_g01_c01[49-64]-[frame12]12.jpg} &


\parbox[c]{4mm}{\multirow{1}{*}[3.5em]{\rotatebox[origin=c]{90}{BB, [0.19]}}} 
\\
\parbox[c]{4mm}{\multirow{1}{*}[4.5em]{\rotatebox[origin=c]{90}{Integrated\cite{integrated}}}} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-2.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-3.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-6.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-7.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-8.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-10.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-12.png} &
% \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-8.png}
\parbox[c]{4mm}{\multirow{1}{*}[3.5em]{\rotatebox[origin=c]{90}{WB, [0.37]}}} 
\\
\parbox[t]{4mm}{\multirow{1}{*}[4.0em]{\rotatebox[origin=c]{90}{STEP\cite{step}}}} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-2.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-3.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-6.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-7.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-8.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-10.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-12.png} &
% \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-8.png}
\parbox[c]{4mm}{\multirow{1}{*}[3.5em]{\rotatebox[origin=c]{90}{BB, [0.87]}}} 
\\
\parbox[t]{4mm}{\multirow{1}{*}[4.0em]{\rotatebox[origin=c]{90}{F-EP (ours)}}} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-2.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-3.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-6.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-7.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-8.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-10.png} &
\includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-12.png} &
% \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-8.png}
\parbox[c]{4mm}{\multirow{1}{*}[3.5em]{\rotatebox[origin=c]{90}{FG, [0.76]}}} 
\\
\end{tabular}
\captionsetup{font=small,aboveskip=3pt}
\caption{\textbf{Visual comparison of explanation methods on the UCF101-24 dataset \cite{ucf101}.} The input (first row) contains consecutive frames from the activity FloorGymnastics. The numbers on the right of each method denote the predicted label and probability for the explanations shown. Compared to other methods, F-EP is able to produce explanations that focus on the foreground person and follow the person's motion.
}
\label{fig:comparison_vis}
\vspace{-10pt}
\end{figure*}


% \newcommand{\framewidth}{0.20\linewidth}

%     \begin{figure}[t]
%     \footnotesize
%     \centering
%     \renewcommand{\tabcolsep}{1.0pt} %
%     \begin{tabular}{ccccc}
%     input & Grad-CAM++ \cite{grad-cam++} & Integrated\cite{integrated} & STEP\cite{step} & F-EP
%     \\
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-2.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gcpp/floorGymnastics_g01_c01[49-64]-2.jpg} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-2.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-2.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-2.png} 
%     \\
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-3.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gcpp/floorGymnastics_g01_c01[49-64]-3.jpg} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-3.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-3.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-3.png} 
%     \\
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-6.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gcpp/floorGymnastics_g01_c01[49-64]-6.jpg} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-6.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-6.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-6.png} 
%     \\
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-7.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gcpp/floorGymnastics_g01_c01[49-64]-7.jpg} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-7.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-7.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-7.png} 
%     \\
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_input/floorGymnastics_g01_c01[49-64]-8.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_gcpp/floorGymnastics_g01_c01[49-64]-8.jpg} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_integrated_grad/floorGymnastics_g01_c01[49-64]-8.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_step/floorGymnastics_g01_c01[49-64]-8.png} &
%     \includegraphics[width=\framewidth]{images/r3d_ucf101/r3d_ucf101_lf_r3/floorGymnastics_g01_c01[49-64]-8.png} 
%     \\
%     29, prob:[0.63] & 14, prob:[0.0004]  & 99, prob:[0.374]   &  4, prob:[0.872]   &   29, prob:[0.760] \\
%     \end{tabular}
%     \captionsetup{font=small,aboveskip=2pt}
%     \caption{\textbf{Comparison of explanation methods on the UCF101-24 dataset \cite{ucf101}.} The input contains 5 frames sampled from a video clip with ground truth Floor Gymnastics. The bottom row for each column denote the predicted label and the predicted probability for each explanation. The explanations of Grad-CAM \cite{grad-cam}, a CAM-based method, are not motion consistent regarding the person's motion. Integrated Grad \cite{integrated}, a backpropagation-based method, produces explanations that are sparse and noisy. The explanations produced by STEP \cite{step} are not motion consistent and focus more on the background sometimes. F-EP (with $r=3$) is able to give spatiotemporal consistent explanations that focus on the person's movements. 
%     }
%     \label{fig:comparison_vis}
%     \vspace{-10pt}
% \end{figure}
